Vision-and-Language Navigation Today and Tomorrow: A Survey in the Era of Foundation Models

Vision-and-Language Navigation (VLN) has gained increasing attention over recent years and many approaches have emerged to advance their development. The remarkable achievements of foundation models have shaped the challenges and proposed methods for VLN research. In this survey, we provide a top-down review that adopts a principled framework for embodied planning and reasoning, and emphasizes the current methods and future opportunities leveraging foundation models to address VLN challenges. We hope our in-depth discussions could provide valuable resources and insights: on one hand, to milestone the progress and explore opportunities and potential roles for foundation models in this field, and on the other, to organize different challenges and solutions in VLN to foundation model researchers.

==> images/category_tree.tex <==
\tikzstyle{my-box}=[
    rectangle,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
]
\tikzstyle{cause_leaf}=[my-box, minimum height=1.5em,
    fill=lighttealblue!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\tikzstyle{detect_leaf}=[my-box, minimum height=1.5em,
    fill=lightplum!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\tikzstyle{mitigate_leaf}=[my-box, minimum height=1.5em,
    fill=harvestgold!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\begin{figure*}[thp]
    \centering
    \resizebox{0.8\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=8pt,
                inner ysep=2.5pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=9.5em,font=\scriptsize,}{},
            where level=2{text width=14.0em,font=\scriptsize,}{},
            where level=3{text width=9.5em,font=\scriptsize,}{},
            where level=4{text width=3.5em,font=\scriptsize,}{},
            [
                \textbf{VLN Agent}, ver, color=pastelblue!100, fill=pastelblue!55,
                text=black
                [
                    \textbf{Past:} \\ LSTM-based VLN Agent (\S Sec:~\ref{sec:past}), color=carminepink!100, fill=carminepink!60, text=black
                    [
                        Multi-modal Explicit Grounding (\S Sec:~\ref{subsec:mmeg}), color=carminepink!100, fill=carminepink!40,  text=black
                    ]
                    [
                        Data Augmentation (\S Sec:~\ref{subsec:da1}), color=carminepink!100, fill=carminepink!40,  text=black
                    ]
                    [
                        Auxiliary Tasks (\S Sec:~\ref{subsec:aux}), color=carminepink!100, fill=carminepink!40,  text=black
                    ]
                    [
                        Map (\S Sec:~\ref{subsec:map}), color=carminepink!100, fill=carminepink!40, text=black
                       % [
                       %     Mapping, color=carminepink!100, fill=carminepink!20, text=black
                       % ]
                       % [
                       %     Planning, color=carminepink!100, fill=carminepink!20, text=black
                       % ]
                    ] 
                    [
                        Outdoor Navigation (\S Sec:~\ref{subsec:outdoor}), color=carminepink!100, fill=carminepink!40,  text=black
                    ]
                    [
                        Dialog/Interactive Navigation (\S Sec:~\ref{subsec:dialog/inter}), color=carminepink!100, fill=carminepink!40,  text=black
                    ]
                ]
                [
                    \textbf{Present:} \\ Transformer-based Agent (\S Sec:~\ref{present}), color=hidden-orange!100, fill=hidden-orange!80, text=black
                    [
                        Large Scale VL Representation Learning (\S Sec:~\ref{subsec:largevl}), color=hidden-orange!100, fill=hidden-orange!40, text=black
                    ]
                    [
                        Data Augmentation (\S Sec:~\ref{subsec:da2}), color=hidden-orange!100, fill=hidden-orange!40, text=black
                        [
                            Pre-training Dataset Augmentation, color=hidden-orange!100, fill=hidden-orange!20, text=black
                        ]
                        [
                            Instruction Augmentation, color=hidden-orange!100, fill=hidden-orange!20, text=black
                        ]
                        [
                            Environment Augmentation, color=hidden-orange!100, fill=hidden-orange!20, text=black
                        ]
                    ]
                    [
                        Graph-based Method (\S Sec:~\ref{subsec:graph}), color=hidden-orange!100, fill=hidden-orange!40, text=black
                    ]
                    [
                        VLN-CE with Waypoint Predictor (\S Sec:~\ref{subsec:vlncewaypoint}), color=hidden-orange!100, fill=hidden-orange!40, text=black
                    ]
                    [
                        Outdoor Navigation (\S Sec:~\ref{subsec:outdoor2}), color=hidden-orange!100, fill=hidden-orange!40, text=black
                    ]
                    [
                        Dialog/Interactive Navigation (\S Sec:~\ref{subsec:dialog/inter}), color=hidden-orange!100, fill=hidden-orange!40,  text=black
                    ]
                    [
                        Analysis Papers (\S Sec:~\ref{subsec:analysis}), color=hidden-orange!100, fill=hidden-orange!40,  text=black
                    ]
                ]
                [
                    \textbf{Future: }\\ LLM-based Agent (\S Sec:~\ref{future}), color=grassgreen!100, fill=grassgreen!70, text=black
                    [
                        LLM Instruction Planner, color=grassgreen!100, fill=grassgreen!40, text=black
                    ]
                    [
                        LLM Navigator, color=grassgreen!100, fill=grassgreen!40, text=black
                    ]
                ]
                [
                    \textbf{Challenges } (\S Sec:~\ref{challenges}), color=lighttealblue!100, fill=lighttealblue!70, text=black
                    [
                        Dataset and Task Challenges, color=lighttealblue!100, fill=lighttealblue!40, text=black
                    ]
                    [
                        Embodied VL Representations, color=lighttealblue!100, fill=lighttealblue!40, text=black
                    ]
                    [
                        LLMs-based VLN Agent, color=lighttealblue!100, fill=lighttealblue!40, text=black
                    ]
                    [
                        Deployment in Real Robots, color=lighttealblue!100, fill=lighttealblue!40, text=black
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{The main categorization of this survey. }
    \label{fig:categorization_of_survey}
\end{figure*}


